ARMOR: Adaptive Curriculum Meta-Learning for Noise-Robust RAG Reasoning

Retrieval-Augmented Generation (RAG) systems have demonstrated remarkable effectiveness in mitigating hallucinations by incorporating external knowledge. However, the retrieval process inevitably introduces noise, posing significant challenges to RAG robustness. Fundamentally, noise robustness is a composite competency encompassing noise identification, retrieval filtering, and robust reasoning. Unfortunately, existing methods often fail to capture this holistic nature, typically restricted to single-dimensional enhancements or hampered by noise-induced optimization interference. To address these limitations, we decompose RAG robustness into three sub-tasks: knowledge boundary perception, retrieval verification, and robust reasoning. Accordingly, we propose ARMOR, an Adaptive Curriculum Meta-Learning for Noise Robust RAG Reasoning. Inspired by the teaching process, ARMOR introduces an adaptive task scheduler as a teacher to curate training plans according to the absolute learning progress of RAG generators (Student). Distinct from GRPO, ARMOR utilizes inter-group advantage estimation during learning to effectively mitigate mode collapse caused by limited output spaces. Experiments on three complex reasoning datasets (2WikiMultiHopQA, MusiQue, and HotPotQA) indicate that ARMOR achieves synergistic improvements in retrieval noise robustness, significantly outperforming baselines in output quality.

==> prompts/method/question-match.tex <==

\begin{figure}[H]
\centering
\setstretch{1.2}
\begin{tcolorbox}[width=0.45\textwidth, title=Prompt for Question Match,
toptitle={0.3em}, bottomtitle={0.1em}]

\textbf{Task Requirements:}

You are an expert at comparing questions. Determine if \textbf{question a} and \textbf{question b} are semantically equivalent (i.e., they ask for the same information and would have the same correct answer). Respond with ONLY ``Yes" or ``No".



\vspace{0.5em}
\textbf{Input:}

	\emph{question a: }\texttt{<}\emph{question a}\texttt{>}
    
    \emph{question b: }\texttt{<}\emph{question b}\texttt{>}


\end{tcolorbox} 
\caption{Prompt for question match.}
\label{fig:Prompt for question match}
\end{figure}



